GeoTP: Latency-aware Geo-Distributed Transaction Processing in Database Middlewares (Extended Version)

The widespread adoption of database middleware for supporting distributed transaction processing is prevalent in numerous applications, with heterogeneous data sources deployed across national and international boundaries. However, transaction processing performance significantly drops due to the high network latency between the middleware and data sources and the long lock contention span, where transactions may be blocked while waiting for the locks held by concurrent transactions. In this paper, we propose GeoTP, a latency-aware geo-distributed transaction processing approach in database middlewares. GeoTP incorporates three key techniques to enhance geo-distributed transaction performance. First, we propose a decentralized prepare mechanism, which diminishes the requirement of network round trips for distributed transactions. Second, we design a latency-aware scheduler to minimize the lock contention span by strategically postponing the lock acquisition time point. Third, heuristic optimizations are proposed for the scheduler to reduce the lock contention span further. We implemented GeoTP on Apache Shardingsphere, a state-of-the-art middleware, and extended it into Apache ScalarDB. Experimental results on YCSB and TPC-C demonstrate that GeoTP achieves up to 17.7x performance improvement over Shardingsphere.

==> sections/cover_letter.tex <==
% \newcommand{\comments}[2]{\noindent{\textbf{Comment #1}}: {#2}}
\newcommand{\response}[2]{\vspace{0mm}\noindent\textbf{Response #1}: {#2}}
\newcommand{\comments}[2]{
% \vspace{4mm}
\noindent\begin{tcolorbox}
[breakable, colback=gray!10, arc=0mm, auto outer arc, boxrule=0pt, boxsep=1pt, before=\vspace{0.5mm}, after=\vspace{0.5mm}]
\noindent\textbf{Comment #1: }
\textit{#2}
\end{tcolorbox}
% \vspace{-1mm}
}

\newcommand{\revhighlight}[1]{\emph{\textbf{\uuline{#1}}}}

\pagestyle{empty}
\thispagestyle{empty}

\newenvironment{figurehere}{%
  \def\@captype{figure}%
  \renewcommand\thefigure{\Roman{figure}}%
  \begin{figure}[!]
}{%
  \end{figure}
}

\newenvironment{bigtablehere}{%
  \def\@captype{table}%
  \renewcommand\thetable{\Roman{table}}%
  \begin{table*}[]
}{%
  \end{table*}
}

\newenvironment{tablehere}{%
  \def\@captype{table}%
  \renewcommand\thetable{\Roman{table}}%
  \begin{table}[]
}{%
  \end{table}
}

% \newcommand{\question}[1]{}
\newcommand{\question}[1]{{\textcolor{blue}{(#1)}}}

\newenvironment{tabhere}{\def\@captype{table}}{}
\makeatletter
\newcommand\figurecaption{\def\@captype{figure}\caption}
\newcommand\tablecaption{\def\@captype{table}\caption}
\makeatother

\renewcommand\thelstlisting{\Roman{lstlisting}}
\twocolumn[\centerline{\textbf{\Large Response to Reviewers' Comments}}\vspace{2mm}]

% \onecolumn

% \centerline{\textbf{\Large Response to Reviewers' Comments}}
\vspace{1mm}

% \begin{multicols}{2}

\setcounter{page}{0}
\setcounter{figure}{0}
\setcounter{table}{0}

\vspace{-2mm}
\noindent We would like to thank the reviewers and meta reviewer for their constructive comments.
We have addressed all the comments in the revised paper. We highlight the major changes made to the manuscript in
{\color{blue} blue}.

\vspace{-2mm}
\section*{Summary of Changes}
\begin{itemize}[leftmargin=*]
% \item We have revised Section~\ref{sec.preliminary.remaster} by, including how to initiate a remaster request and how to reach a consensus on remastering.

\item We have made the source code of \dbname publicly available at \url{https://github.com/dbiir/GeoTP}.

\item We have revised Section \ref{intro} and Section \ref{sec.related} to discuss the related works mentioned by reviewers.

\item We have improved Section \ref{intro} to clarify the motivation and novelty of the decentralized prepare mechanism, which is designed to optimize performance for general transactions, including interactive transactions and stored procedures.
% In particular, we have enhanced the description to make the explanation of distributed transaction processing more general, rather than only "single-stage" transactions.

\item We have updated Section \ref{design-3} and Section \ref{design.discussion} to clarify \dbname's assumptions and discuss heuristic optimizations for handling inaccuracies in the prediction model.

\item We have substantially enhanced the experiments in Section \ref{sec.evaluation} according to the reviewers' constructive comments. \blackding{1} We have enhanced the description of the default configuration, baselines, and benchmarks in Section \ref{sec.evaluation.setup}. 
\blackding{2} We have improved Section~\ref{sec:evaluation_scalability} to analyze the overhead of \dbname, covering CPU utilization, memory usage, and a breakdown of each key module on the critical path of distributed transactions. 
\blackding{3} We have enhanced Section \ref{sec:evaluation_workloads} and Section \ref{sec:evaluation_optimization} to analyze the tail latency of \dbname and each baseline. 
% the latency distribution under different contention scenarios in Figure~\ref{Fig.experiment.ycsb.ds.cdf} .
\blackding{4} We have updated Section \ref{sec:evaluation_optimization} to illustrate the abort rate under different contention workloads and analyzed the impact of each \dbname's optimization on it. 
\blackding{5} We have revised Section \ref{sec.eva.heterogeneous} to strengthen the experiments on heterogeneous scenarios, demonstrating the effectiveness of \dbname's optimizations. 
\blackding{6} We have revised Section \ref{sec:evaluation_yugabyte} to clarify YugabyteDB's optimizations for ``single-row/single-shard" transactions and to highlight how these differ from those in \dbname. 
\blackding{7} We have added Section \ref{sec:evaluation_length} to provide a detailed evaluation of \dbname's performance with transactions of various lengths and multiple interactive rounds.
\blackding{8} We have evaluated the deployment where \dbname is deployed on different regions to further test its scalability; due to space limitations, we leave it in the extended version~\cite{GeoTP}. 

\item To make space for the above changes, we have moved the algorithm of the first optimization, the illustration example of early abort previously in Section \ref{design-1}, the discussion of the integrity constraint problem previously in Section \ref{design-3}, and part of the failure recovery description previously in Section \ref{sec.failure} to the extended version~\cite{GeoTP} and tried our best to make sure that these sections remain concise. 
% We have tried our best to make sure that these sections remain concise, and their fuller versions can be found in the extended manuscript~\cite{GeoTP}.

\end{itemize}


% \vspace{-2.5mm}
\section*{Response to Meta-Reviewer}

\comments{Meta.1}{Ensure artifacts can be accessed}

\response{Meta.1}{
We have made the source code of \dbname publicly available at \url{https://github.com/dbiir/GeoTP}.
}

\comments{Meta.2}{Discuss the similarities and differences to related works mentioned by reviewers}

\response{Meta.2}{
% We have read the related work~\cite{DBLP:conf/eurosys/ChenSJRLWZCC21}, which presents DAST, an edge database that can meet stringent performance in geo-distributed scenarios. DAST also considers the network latencies difference between inner-region and outer-region nodes and then allocates an appropriate further timestamp for distributed transactions from blocking other transactions. However, it does not reduce the network round trips for distributed transactions, and it ignores the network latency difference within outer-region nodes and the execution latency in high contention workloads. Moreover, the transaction processing model in the edge database is different from it in the database middleware. Hence, its optimizations can not be utilized directly. 
We have revised Section \ref{intro} and \ref{sec.related} to include the related works mentioned by the reviewers.
% zh todo We have added expriments
Please kindly refer to our response to R1O2 for more details.
}

\comments{Meta.3}{Clarify the transaction structure in experiments, and impact of varying transaction length}

\response{Meta.3}{
Following your suggestions, we have clearly stated the experimental settings for the transaction structure in Section~\ref{sec.evaluation.setup} and further evaluated the impact of transaction length in Section \ref{sec:evaluation_length}.
% in Figure \ref{Fig.experiment.length}
% transaction structure used in our experiments, we extend the YCSB+T benchmark to simulate various transactional workloads, where the transactions include 5 operations by default, which have a 50 percent probability of read or write operation.
% We have enhanced our evaluation to illustrate the impact of transaction round and transaction length in Figure \ref{Fig.experiment.length} and revised Section \ref{sec:evaluation_scalability}. 
Please refer to our responses to R1O1, R2O3, and R3D1 for more details.
}

\comments{Meta.4}{Be explicit about the assumptions eg knowing read and write sets (knowing read sets can be problematic with predicate-based selection and phantom issues, except if a key-value model is assumed)}

\response{Meta.4}{
We have revised Section~\ref{sec.overview} to clarify our assumptions. 
We assume that applications can use annotations, which are prefixes or suffixes on SQL statements, to pass certain operation hints to \dbname.
Given that SQL annotations are commonly used to manually guide and influence database query optimization, we consider this assumption to be reasonable.
In \dbname, we employ these annotations to indicate the last operation in the proposed decentralized prepare mechanism.
Further, we have enhanced Section \ref{design.discussion} to clarify that \dbname does not require the read and write sets to be known in advance. 
Please refer to our responses to R1O3 for more detailed explanations.
% There are no phantom issues because the isolation guarantee is provided by the concurrency control algorithms of each data source.  
% Most queries or updates target the primary key, allowing the read/write records to be inferred from the predicate. 
% This helps identify hotspot data and estimate sub-transaction execution time. 
% To enhance efficiency, we use an AVLTree to organize hotspot data Meta.information, achieving O(log n) complexity for queries and modifications. 
% For non-primary key queries, \dbname's heuristics optimization will ignore them. 
% Additionally, \dbname's other two methods remain effective and continue to optimize performance in this scenario. 
}

\comments{Meta.5}{Improve discussion of first optimisation so motivation is clear}

\response{Meta.5}{
We have revised Section \ref{intro} to strengthen the motivation of the first optimization. 
In typically distributed transaction processing, a transaction first performs read/write operations during the execution phase and then employs a two-phase commit, which includes a prepare phase and a commit phase, to ensure atomicity \cite{DBLP:journals/pvldb/ZhangLZXLXHYD23}. 
The prepare phase, in particular, is on the critical path of transaction processing and can thus become
a significant performance bottleneck.
% Since database middleware must handle various transaction protocols from different data sources, eliminating the prepare phase is not straightforward. 
To address this, \dbname introduces a decentralized prepare mechanism to reduce network round trips of the prepare phase, thereby improving transaction performance.
Please refer to our response to R1O1 for more detailed clarifications.
% In particular, we design an efficient component to abstract the differences of data sources, and propose an early abort mechanism 
% reduce WAN communication costs, thereby enhancing performance in geo-distributed database middleware. 
% In addition, a transaction may include multiple read/write operations, which can incur several rounds of network communications during the execution phase. 
% We have conducted evaluations that encompass various transaction lengths and interaction scenarios. 
% The latency requirements for interactive transactions are generally less stringent~\cite{DBLP:conf/usenix/CowlingL12, DBLP:journals/pvldb/KallmanKNPRZJMSZHA08}. 
% Transactions derived from application APIs or stored procedures involve a few interactive rounds. In such scenarios, minimizing WAN communication costs is crucial.
% Furthermore, existing solutions typically require protocol modifications within the database kernel, making them impractical for middleware scenarios that need to handle heterogeneous databases. To address this, \dbname introduces a lightweight yet effective component called Geo-agent to mask the difference between database engines.
% Lastly, we have conducted evaluations to cover various transaction lengths and interaction scenarios.
% , as shown in Figure~\ref{Fig.experiment.length}. Although \dbname's performance gains decrease as the number of interactions and transaction lengths increase, it still significantly outperforms the baseline. 
}

\comments{Meta.6 (Optional)}{Explore varying the latency assumptions}

\response{Meta.6}{
% \dbname is designed to enhance transaction performance for database middleware in geo-distributed environments, where network latency between the middleware and database nodes is prolonged and highly variable. 
Following your suggestion, we have simulated various network latencies between the middleware and data sources and explored the performance of \dbname over different network configurations, to assess how network latency affects system performance.
Please refer to our response to R2O2 for more detailed analysis.
}

\comments{Meta.7 (Optional)}{Show/discuss abort rates and tail latencies in experiments}

\response{Meta.7}{
As required, we have updated Figure \ref{Fig.experiment.ycsb.skew} to include the abort rates and updated Figure \ref{Fig.experiment.ycsb.ds.cdf} and Figure \ref{Fig.experiment.ycsb.skew} to show tail latencies. We have added the corresponding discussion in Section \ref{sec:evaluation_workloads} and Section \ref{sec:evaluation_optimization}.
Please refer to our responses to R1O4 and R2O4 for more detailed clarifications.
}


% We have addressed all the required changes accordingly. 
% Please kindly refer to our responses to R1, R2, and R3 below for details.

% \revision{We summarize our changes below:}

% {\color{red}
% Provide a summary of changes -- new experiments and systems for comparasion, and then
% respond as with others -- concise and the refer to the R\#Q\# in the response to others for details}.

% \ensuremath{\texttt{\dbname}\xspace}



% \vspace{-2mm}
\section{Response to Reviewer \#1}
\comments{O1}{The first problem of over-coordination is not clear. Somehow it is hinted that the typical case of coordination in DB middleware is to employ a 3PC (execution, prepare, commit). However, most “textbook” distributed serializable DBs employ a 2PC since lock+execute suffices for phase-1 and then final commit in phase-2, e.g. when used in conjunction with 2PL for locking-unlocking. My confused guess (since this is not disclosed clearly in the paper) is that execution (phase 1) entails a regular 2PL (through preparing txn statements) over different stages of the query, and coordination is needed at the end to communicate to all DS that all stages are clear, initiating 2PC to commit the change log. Now, the example discussed in Fig.3 is already a “single-stage” transaction, so it is trivial to run prepare right after, but how about multi-stage transactions with complex dependencies? Is there something novel done here that I don’t see? I think the motivation needs to be updated to better showcase this contribution.}

\response{O1}{
% we aim to develop a general-purpose middleware capable of  transactions, such as interactive transactions and stored procedures.
We would like to clarify that for general transactions, whether interactive or stored procedures, the typical distributed transaction processing protocol~\cite{DBLP:journals/pvldb/ZhangLZXLXHYD23} first executes read/write operations during the execution phase, followed by two-phase commit (2PC), including a prepare phase and a commit phase, to ensure transaction atomicity.
It is widely recognized that 2PC, particularly the prepare phase, is on the critical path of transaction processing and can thus become a significant performance bottleneck~\cite{DBLP:journals/pvldb/ZhangLZXLXHYD23, DBLP:journals/pvldb/MaiyyaNAA19, DBLP:conf/sosp/ZhangSSKP15}. 
To optimize transaction performance, we are therefore motivated to reduce the costs associated with the prepare phase while ensuring that \dbname supports general-purpose transactions.
In particular, we propose a decentralized prepare mechanism, which allows the prepare phase to begin immediately after the completion of local execution.
This mechanism offloads the coordination
cost from the middleware and eliminates one WAN round trip, thereby reducing the latency of distributed transactions.
However, performing decentralized prepare across diverse data sources is challenging due to the varied transaction protocols they employ.
Unlike existing solutions~\cite{DBLP:journals/pvldb/MaiyyaNAA19, DBLP:journals/pvldb/ZhangLZXLXHYD23, DBLP:conf/sosp/ZhangSSKP15, DBLP:conf/usenix/CowlingL12} in distributed database systems, which typically rewrite the transaction protocol, we introduce a non-intrusive and lightweight decentralized prepare mechanism for the middleware system.
We leverage annotations, supported by most data sources, to mark the last read/write operation and develop an efficient component called geo-agent to abstract differences between data sources, thereby enabling decentralized preparation across various systems.
In addition, we design an early abort mechanism that allows fault transactions to abort quickly, preventing such transactions from degrading system performance. 
We have improved Section~\ref{intro} to clearly articulate the motivation and novelty of the proposed decentralized prepare mechanism and better explain the typical distributed transaction processing protocol.
% Further, \dbname. 
% and enable the communication of different kinds of data sources to reduce the coordination cost both in the prepare stage and in the rollback scenarios. 
% {\color{blue}
% Second, in the event of errors during the prepare phase, our early abort mechanism enables the faulty data source to directly notify other involved peers without middleware coordination. Additionally, we design a failure recovery mechanism to ensure the correctness of transaction processing under the decentralized prepare mechanism.
% }

% , we redesign the failure recovery protocol to keep consistency when encountering either middleware failure or data source failure.
% makes them different from applying in the middleware, where they need to handle heterogeneous data sources with different transaction processing protocols. 

We understand that a transaction may include multiple read/write operations, which can incur several rounds of network communications during the execution phase.
We have conducted additional experiments 
to evaluate how \dbname performs as the number of network communication rounds increases in the execution phase.
The results, presented in Figure~\ref{Fig.experiment.length}, show that as the network round trips increase from 1 to 6, the performance of \dbname decreases by 44.3\% and 82.0\% in low and medium contention workloads.
However, \dbname still outperforms the baselines by up to 3.4x due to the decentralized prepare mechanism and latency-aware scheduling. 
Further, it is important to note that most real-world distributed transactions tend to minimize execution round trips for better performance. 
For example, standard transactions, such as transferring balance between user accounts and updating user profiles in web applications~\cite{DBLP:conf/sigmod/YangY022, DBLP:conf/sigmod/Pavlo17} require just two rounds for execution: the first round retrieves all the necessary reads, followed by a second round for the writes~\cite{DBLP:conf/eurosys/ChenSJRLWZCC21}. 

% Transactions can decide the write values based on the read results. 
% Interactive transactions usually include multiple interactive rounds but don't have low latency requirements~\cite{DBLP:conf/usenix/CowlingL12, DBLP:journals/pvldb/KallmanKNPRZJMSZHA08}.

% contains multiple stages for execution and two for prepare and commit. 
% The ``textbook" 2PC protocol contains the prepare stage and commit stage. 
}

% Transactions derived from application API or stored procedure typically don't involve many interactive round trips \cite{DBLP:conf/eurosys/ChenSJRLWZCC21}. Furthermore, Carousel proposed the 2FI transaction model, which executes transactions in two rounds: a read round followed by a write round. Transactions can decide the write values based on the read results. 
% % This interactive read-write pattern between clients and servers is preferred by many applications, and m
% Many transactions can fit in the 2FI model, including transferring balance between user accounts and updating user profiles in web applications~\cite{DBLP:conf/sigmod/YangY022, DBLP:conf/sigmod/Pavlo17}. 
% In these transactions, reducing the overhead of 2PC has a large improvement in transaction performance. 
% Although there are multiple solutions to eliminate the cost of 2PC in distributed database systems, the requirement of rewriting the transaction protocol makes them different to apply in the middleware, where they need to handle heterogeneous data sources with different commit protocols. 




% 1. different 3 phases， 我们说的是提交和运行; 2. 我们的目的是消除 prepare，这是一个起点; 3. 怎么把 prepare 消除掉，已有的工作，我们提出了一个巧妙的

\comments{O2}{Regarding the second problem, I am worried that delayed scheduling/locking has been explored numerous times before in slightly different setups. For example, [Chen] from EuroSys ’21 presents a very similar idea in the context of edge transactions, yet not cited or discussed in this paper. The related work focuses primarily on middleware and not-so-related approaches such as TAPIR.}

\response{O2}{
Following your suggestion, we have revised Section \ref{intro} and Section \ref{sec.related} to include related works on delayed scheduling/locking techniques. 
DAST~\cite{DBLP:conf/eurosys/ChenSJRLWZCC21} is designed to meet the performance requirements of edge database systems. 
It categorizes transactions into intra-region and cross-region transactions, assigning a larger timestamp to cross-region transactions to allow faster processing of intra-region transactions. However, DAST overlooks network latency differences between nodes in different regions, which limits its ability to optimize cross-region transactions.
% For example, the round-trip time from Beijing to Shanghai is 27 ms, while it is 73 ms to Singapore. 
% For a transaction involving both nodes, DAST's delayed scheduling may lock records in Shanghai for 73ms. 
Further, several scheduling techniques have been proposed for distributed databases.
QURO~\cite{DBLP:journals/pvldb/YanC16} reorders operation sequences and delays exclusive lock acquisition, but it does not consider latency variations across nodes in different regions as well.
Chiller~\cite{DBLP:conf/sigmod/ZamanianSBK20} shares a similar idea with DAST, and therefore, it faces the same limitations as DAST.
% In addition to DAST's limitations, 
% Chiller can further increase distributed transaction latency by waiting to schedule inner-region subtransactions until the outer-region is complete. 
Unlike these works, \dbname introduces a latency-aware scheduling technique that operates in a fine-grained manner, enabling precise identification of the most appropriate scheduling for each operation.
We have also conducted additional experiments to demonstrate the performance gains of \dbname compared to these approaches.
Please refer to our response to R3O2 for more details.
}
% deferring the inner part until after the outer-region part to reduce lock contention, as the inner part often involves hot records. 
% Further, \dbname reduces WAN communication costs in distributed transactions, addressing a major bottleneck in geo-distributed scenarios.

% considers network latency differences across all nodes involved and local execution latency, allowing for finer precision.
% in high-contention workloads. 
% DAST can not be directly applied in database middleware due to differences in transaction processing models. 
% separates intra-region transactions (IRT) from cross-region transactions (CRT) 
% Moreover, there are some related work about delayed scheduling/locking. 
% DAST takes into account the network latency differences between inner-region and outer-region nodes, allocating appropriate timestamps for distributed transactions to prevent blocking other transactions. However, the edge database technique used by DAST operates on a different transaction processing model compared to \dbname, making its optimizations unsuitable for direct application in database middleware.
% Moreover, \dbname reduces WAN communication costs for distributed transactions and provides a more detailed exploration of the challenges and opportunities for improvement due to network differences. 


\comments{O3}{The third and last technique on high-contention workload optimisations is expanding the idea of delayed transactions with workload analysis and I find this interesting. Nevertheless there is a catch too here that is not discussed at all in the paper and that is the implicit need to know apriori the read-write sets of the transactions. This is a quite strong compromise here that contradicts the goal of a general-purpose DB middleware. A good discussion on this is more than welcome.}

\response{O3}{
We would like to clarify that \dbname does not require the read-write sets of transactions to be known in advance. 
Instead, we identify hotspot records based on given query statements for the proposed high-contention optimization.
In particular, when a user specifies a predicate on the primary key or a key from a secondary index, we identify hotspot records that match the predicate and then estimate the local execution latency of sub-transactions on them.
% the primary key of the records can be derived from the query predicates or query plans after traversing the secondary index.
% Using these keys, we identify hotspot data and estimate the local execution latency of sub-transactions.
% To enhance efficiency, we use an AVLTree to organize hotspot data Meta.information, achieving O(log n) complexity for manipulation.
% We acknowledge that in some cases, such as range queries, the primary key cannot be inferred from the operation statements, which may limit the effectiveness of this technique.
We acknowledge that in certain cases, such as when there is no index on the predicate key, inferring hot records from the statements is challenging, and therefore, the proposed high-contention optimization can be ineffective. 
However, since most transactional workloads~\cite{TPCC, DBLP:conf/icde/AlomariCFR08} either access primary keys or use index searches for improved efficiency, such ineffective cases are relatively rare.
Moreover, even when this high-contention optimization is ineffective, \dbname is not compromised. 
Other optimizations, such as latency-aware scheduling, continue to enhance performance, as demonstrated in our ablation study in Section \ref{sec:evaluation_optimization}. 
% zh: nothing changed in Section 2?
We have revised Section \ref{design-3} and Section \ref{design.discussion} to incorporate these discussions for better clarity.
% For queries or updates targeting the primary key, which is common in transactional workloads, the read/write records or intervals can be inferred from the predicate. 
% This inference helps identify hotspot data and estimate sub-transaction execution times, allowing for the appropriate delay of corresponding sub-transactions. 
% For non-primary key queries, \dbname's heuristic optimization will ignore them. Nonetheless, \dbname's other two optimization methods remain effective and continue to enhance performance in such scenarios. 
% We have revised Section \ref{design-3} to discuss the application scope of the third optimization. 
}


\comments{O4}{I do not have many concerns regarding the evaluation results. It would be fair to show more detailed latency plots, such as 99-percentile latencies. It is OK to show and discuss the penalties of certain delayed queries, especially during high contention. This can boost the credibility of your results.}

\response{O4}{
To address your concern, we have provided the latency distribution under different contention scenarios in Figure \ref{Fig.experiment.ycsb.ds.cdf}. 
We can observe that the 99th-percentile (p99) latency of \dbname is up to 35.9\% lower than that of baselines across all contention scenarios, demonstrating its superior performance.
In the high contention scenario, however, while \dbname maintains a lower p99 latency, its advantage in p99.9 latency diminishes. 
This is due to the proposed high-contention optimization, which may result in additional aborts. 
However, this increased tail latency only affects a small portion of transactions, while the overall throughput improves with the high contention optimization.
We have also included p99 latencies in Figure~\ref{Fig.experiment.ycsb.skew}, which further demonstrate the performance advantages of \dbname compared to baselines.
% and \dbname's p95 latency remains well below that of the baselines.
% We highlighted Section \ref{sec:evaluation_workloads}
% Following your advice, 
% and enhanced Section \ref{sec.eva.heterogeneous} to include the p99 latencies. 
}

\section{Response to Reviewer \#2}

\comments{O1}{Comparison mainly against the very Apache Shardingsphere system on which the actual implementation is based on.}

\response{O1}{
We would like to clarify that in our initial submission, we mainly evaluated \dbname against ShardingSphere to ensure fair comparisons.
Since \dbname is implemented based on the codebase of ShardingSphere, we opt not to directly compare it with other middleware systems due to differences in foundational codebases.
However, we integrate our proposed techniques from \dbname to ScalarDB (denoted as ScalarDB+).
The results, shown in Figure \ref{Fig.experiment.sca}, demonstrate the general applicability of our proposed techniques to other middleware systems.
In addition, following the suggestion from R3O2, we have conducted additional experiments to compare \dbname with two related approaches, QURO~\cite{DBLP:journals/pvldb/YanC16} and Chiller~\cite{DBLP:conf/sigmod/ZamanianSBK20}. 
To ensure fair comparisons, we implemented both approaches on the same platform as \dbname.
As shown in Figure~\ref{Fig.experiment.ycsb.ds} and Figure \ref{Fig.experiment.tpcc.dis}, \dbname outperforms QURO and Chiller over both YCSB and TPC-C benchmarks.
Please kindly refer to our responses to R3O2 for more details.
% We have revised Section \ref{sec:evaluation_workloads} to improve the comparison against other approaches. 
}
% We have included two related approaches, QURO~\cite{DBLP:journals/pvldb/YanC16} and Chiller~\cite{DBLP:conf/sigmod/ZamanianSBK20} in our experiments, as pointed out in R3O2.
% Both approaches aim to reduce lock contention: QURO reorders the operation sequence in application code and delays the write operations, while Chiller divides transaction execution into inner- and outer-region parts, executing the inner part after the outer-region part to minimize lock contention, as the inner part typically involves hot records. 


\comments{O2}{The experimental evaluation uses a fixed setup of simulated geo-distributed database nodes always consisting of four database nodes, one very fast local node (0 ms latency), two regional nodes with medium latency of 27ms and 73ms, and one inter-continent latency of 251ms. How do these latencies relate to the variations measured in Section VII.D? How would the systems scale with a larger number of nodes or only wide-area nodes?}
% 27 73 是实际测出来的， 
% 时延，中间件，

\response{O2}{
\begin{table}[]
\centering
\caption{Network latency configurations}
\label{Tbl.revise.network}
\begin{tabular}{ccccccccc}
\Xhline{2pt}
\multirow{2}{*}{Node count}  & \multicolumn{8}{c}{Latency from DM to data sources (ms)} \\ \cline{2-9} 
       & \#1   & \#2   & \#3   & \#4  & \#5  & \#6  & \#7  & \#8  \\ 
\Xhline{2pt}
4 nodes & 0     & 27    & 73    & 251  & -    & -    & -    & -    \\ \hline 
5 nodes & 0     & 27    & 73    & 251  & 0    & -    & -    & -    \\ \hline 
6 nodes & 0     & 27    & 73    & 251  & 0    & 13   & -    & -    \\ \hline
7 nodes & 0     & 27    & 73    & 251  & 0    & 13   & 50   & -    \\ \hline 
8 nodes & 0     & 27    & 73    & 251  & 0    & 13   & 50   & 162  \\ 
\Xhline{2pt}
\end{tabular}
\end{table}
% is the default network configuration, which is measured in the geo-distributed deployed servers. 
We measure the real network latency on Aliyun ECS~\cite{ecs}, and set this as the default network configuration.
To further assess how network latency affects system performance, we simulate various network latencies between the middleware and data sources and explore the performance of \dbname over different network configurations in Section \ref{sec:evaluation_dynamic_network}. 
Specifically, we first investigate the impact of absolute network latency by adjusting the mean latency between the middleware and data sources while keeping their standard deviation stable.
We then evaluate the effect of the network latency variation among different data nodes by fixing the mean latency but varying the standard deviation.
Please note that this set of experiments includes the scenario where all data nodes are located in wide-area networks.
For example, when the mean latency is set to 20ms, the latencies between the middleware and three data nodes are 10ms, 20ms, and 30ms, respectively.
We have revised  Section~\ref{sec.evaluation.setup} to clarify the default network configuration and improved Section \ref{sec:evaluation_dynamic_network} to present the performance evaluation under various network latency configurations more clearly.


Following your suggestion, we have also conducted additional experiments with the number of data nodes increasing from 4 to 8.
The network latencies of different settings are listed in Table \ref{Tbl.revise.network}. 
As shown in Figure \ref{Fig.revise.node}, the performance gains of \dbname remain relatively stable across different node counts.
This observation indicates that in geo-distributed scenarios, network latency has a greater impact on transaction performance than the number of nodes. 
In other words, if the network latency involved in a transaction gets smaller, performance can scale up as nodes increase. 
Due to space constraints, we opt to include Figure \ref{Fig.revise.node} in the extended version of our paper~\cite{GeoTP}. 


\begin{figurehere}
    \centering
    \includegraphics[width=0.25\textwidth]{figures/evaluations/revision/node_cnt.pdf}
    \vspace{-1mm}
    \caption{Impact of node numbers over YCSB}
    \label{Fig.revise.node}
    \vspace{-4mm}
\end{figurehere}
}

\comments{O3}{Most experiments use the YCSB benchmark which be default is not transactional, even though some operations might access multiple records. The mapping to transactions in this paper, hence, is not fully defined. Why not use the YCSB+T benchmark variant which beyond defining meaningful transactional boundaries that would suite the use-case here also would allow to check for the correctness of the executions at the end?}

% 我们的 YCSB 指的是 YCSB+T；我们 YCSB+T 在我们场景下存在的问题，。。。
\response{O3}{
\begin{tablehere}
\caption{Evaluation over YCSB+T}
\label{Tbl.revise.ycsbt}
\vspace{-2mm}
\resizebox{\linewidth}{!}{
\begin{tabular}{llll}
    \Xhline{2pt}
      & Throughput (Txn/s) & Average latency (ms) & P99 latency (ms) \\
    \Xhline{1pt}
SSP   & 88.4               & 972.0                & 2445.3                      \\
GeoTP & 345.8              & 222.8                & 1267.7                    \\
    \Xhline{2pt}
\end{tabular}
}
\end{tablehere}
We would like to clarify that we employ a YCSB variant inherited from existing works~\cite{DBLP:journals/tkde/ZhaoZZLLZPD23, DBLP:conf/icde/ZhengZLYCPD24}.
In this benchmark, each transaction contains 5 operations by default, with a 50 \% probability of either read or write operation.
We have clarified the details of our YCSB benchmark in Section \ref{sec.evaluation.setup} to eliminate ambiguity. 
Following your suggestion, we have also conducted additional evaluations using YCSB+T under medium contention.
As listed in Table \ref{Tbl.revise.ycsbt}, \dbname outperforms SSP by 3.9x, demonstrating similar trends to those observed in our experiments with the YCSB variant.

% To conduct more fine-grained experiments, we chose to 
% We extend them in our evaluation to compare and explore performance in various workloads, where e
}

\comments{O4}{Abort rates are not reported which would be interesting given that one of the optimisations allows some sub-transactions to abort early.}

\response{O4}{
We have enhanced Figure \ref{Fig.experiment.ycsb.skew} to include the corresponding abort rate.
The results show that even in a high-contention scenario (skew factor set to 1.7), \dbname achieves a 23.4\% reduction in aborts compared to SSP.
This improvement is attributed to our high-contention optimization, which efficiently schedules transactions to execute during periods of lower conflict, thus reducing abort rates.
Regarding the high-contention optimization (O3), we observe an 8.5\% increase in the abort rate compared to \dbname (O1$\sim$O2), but it yields 1.7x higher throughput and 8.6\% lower latency.
This is due to the fact that O3 strategically aborts some transactions to relieve contention, allowing retries during less congested periods.
While this raises the abort rate slightly, it enables more precise scheduling by considering the local execution time, further reducing the lock contention span and improving overall performance. 
% that while it increases the abort rate by 8.5\% compared to \dbname (O1$\sim$O2), it also results in 1.7x higher throughput and 8.6\% lower latency. 
% ...[1. why abort rate increases 2. why performance increses]
We have revised Section \ref{sec:evaluation_optimization} to incorporate this discussion on abort rates, providing better clarity on the advantages of our proposal and a deeper understanding of the high-contention optimization.
% does not significantly increase the abort rate since before \dbname chooses to block the transaction, it tries to block several times and allows execution if there is less conflict between it and concurrent transactions. 
% The results, xxx
% Add the abort rate in Table heterogeneous scenarios 
}

\comments{C1}{In Section VII.B (Evaluation of Overall Performance of GeoTP), what is exactly measured here? Is this with the default values of 20\% distributed transactions and 80\% local tx on medium contention for YCSB? This is not quite clear from the overall and quite detailed description of the experimental setup.
Similar at section VII.C - how many terminals are used here?}

\response{C1}{
In Section \ref{sec:evaluation_scalability}, we evaluate the performance of \dbname by varying the number of client terminals over YCSB and TPC-C benchmarks. 
We use the default settings of YCSB, as specified in Section \ref{sec.evaluation.setup}, which consist of 20\% distributed transactions and 80\% centralized transactions under medium contention. 
In Section \ref{sec:evaluation_workloads}, the number of terminals is set to 64, which is the default configuration.
We have stated these default configurations more clearly in Section \ref{sec.evaluation.setup}. 
}

\comments{C2}{Why the separation of the throughput results of ScalarDB/ScalarDB+ from SSP and GeoTP? Is this to not mix the two different base implementations (SSP/ScalarDB)? The corresponding description should explain this briefly and also remind us which optimisation techniques from GeoTP have been implemented in ScalarDB+.}

\response{C2}{
We chose not to directly compare \dbname with ScalarDB due to differences in foundational codebases.
% We separately discuss the performance of SSP and ScalarDB because they obey different middleware architectures. Direct comparison is unfair. 
In contrast, we integrate our proposed techniques into ScalarDB, denoted as ScalarDB+.
Following your suggestion, we have enhanced Section \ref{sec:evaluation_scalability} to clarify that we compare ScalarDB and ScalarDB+ to demonstrate the effectiveness and generality of the proposed techniques and revised Section \ref{sec.evaluation.setup} to add the explanation of ScalarDB+.
}

\comments{C3}{Section VII.C (Impact of Distributed Transactions): GeoTP also seems to have a turning point around 40\% distributed transactions, at least for the medium contention case, though less pronounced than with SSP... (the text claims there are none)}

\response{C3}{
% \todo{}
\dbname has a ``turning point" around 40\% in the medium contention since the distributed transactions ratio is 0.6. The turning point implies that the optimizations of \dbname can significantly reduce the lock contention span and reduce the negative impact of distributed transactions on centralized transactions. 
We have revised Section \ref{sec:evaluation_workloads} to explain the turning point in medium scenarios.
% We have added some explanation on in Section \ref{sec.evaluation}
}

\comments{C4}{Section VII.F (Impact of Heterogeneous Databases): From the experimental description at the start of this section it becomes not clear that nodes N1 and N2 have presumably much faster network latencies than nodes N3 and N4 (at least according to the experimental setup given at the beginning of VII). This seems to be the main driver of the differences in measured tx latencies in this experiment (Table I). So is this more an experiment to compare latencies rather than database systems?}

\response{C4}{
We have revised Section \ref{sec.eva.heterogeneous} to enhance the experiments on heterogeneous scenarios. 
The network latency from DM to data sources, denoted as $N_1\sim N_4$, are 0, 27 ms, 73 ms, and 251 ms, respectively, and we keep them constant to evaluate data source variations. 
% We fix the network latency to evaluate the data source differences. 
We have updated the deployment scenarios to make our experiments focus on assessing the performance of different underlying data sources, rather than the impact of varying latencies.
In particular, we have conducted experiments on three new deployment scenarios: (a) MySQL is deployed on nodes {\small $N_1 \sim N_4$}; (b) PostgreSQL is deployed on nodes {\small $N_1$ \& $N_3$}, and MySQL is deployed on nodes {\small $N_2$ \& $N_4$}; (c) PostgreSQL is deployed on nodes {\small $N_1 \sim N_4$}. 
% (a) four MySQL servers, (b) two MySQL servers and two PostgreSQL servers, and (c) four PostgreSQL servers. 
As shown in Table~\ref{Tbl.experiment.heterogeneous}, the throughput improvement of \dbname ranges from 3.6x to 7.5x, with the average latency reduction varying between 62\% and 87.8\%. 
The evaluation result can prove that (1) both MySQL and PostgreSQL suffer from prolonged network latency in geo-distribution scenarios; (2) \dbname's optimizations are generally applicable for different data sources and can improve the performance in these scenarios.
% Please refer to Section \ref{sec.eva.heterogeneous} for more details.
}

\comments{C5}{
Comparison with YugabyteDB: How differs the mentioned performance optimisation for "single-row/single-shard transactions" in YugabyteDB from the dedicated handling of centralised transactions in GeoTP?
}

\response{C5}{
We have revised the text in Section \ref{sec:evaluation_yugabyte} to state the difference between \dbname and YugabyteDB more clearly.
YugabyteDB simplifies its transaction commit logic through optimizations in its database kernel.
Specifically, for single-row or single-shard transactions, it can perform data updates asynchronously after the transaction is committed.
In contrast, \dbname, which does not directly modify the underlying data source, typically lacks this optimization.
In low-contention workloads, where transaction contentions no longer dominate performance, the performance gap due to these fundamental codebase differences of \dbname and YugabyteDB becomes more apparent.
However, \dbname can also benefit from the asynchronous data update if the underlying data source supports this technique.
Therefore, we consider this technique to be orthogonal to our proposal.
% During execution, it writes provisional records for each participant, and in the commit phase, it accesses the transaction status table with a single WAN round trip while applying the provisional records asynchronously. 
% Additionally, single-row or single-shard transactions bypass the transaction status table, reducing network communication even further.
% {\color{red} YugabyteDB optimizes single-row/single-shard transactions by bypassing updates to the transaction status table}, which reduces network communication and accelerates these transactions compared to distributed ones. 
% Furthermore, YugabyteDB’s use of multi-version concurrency control (MVCC) enables concurrent read and write operations, boosting performance in low-contention workloads. However, adopting MVCC in \dbname would increase complexity and the cost of ensuring serializability, as it would require consistent snapshot management and global dependency ordering.
}

\comments{C6}{
The nodes used in the evaluation, are they actually five separate servers or VMs that reside in the four cities mentioned, or are they `simulated' nodes via a local cluster with simulated network latencies?
}
% highlight 了

\response{C6}{
The nodes used in the evaluation are five separate servers in a local cluster.
We simulate their network latencies using the \textit{tc} command provided by Linux.
We measure the real network latency on Aliyun ECS~\cite{ecs}, and set this as the default network configuration.
% The latencies between Beijing and the other three sites are tested in the real cloud environment, i.e., Aliyun ECS.
We have improved Section \ref{sec.evaluation} to clarify these statements.
}

\section{Response to Reviewer \#3}
\comments{O1}{
GeoTP's optimizations are rather simplistic. For example, starting the first phase of 2PC on the last update is a rather straightforward optimization. The trick in this paper was to push an annotation to the database to let it know that it was the last update. This requires a somewhat invasive application change.
}

\response{O1}{
% \todo{}. Rewrite the motivation of the first contribution
% As stated in our response to Meta.4, we assume that applications can use annotations, which are prefixes or suffixes on SQL statements, to pass certain operation hints to \dbname.
We would like to clarify that SQL annotations are commonly used to manually guide and influence database query optimization~\cite{MySQL_Hint, PostgreSQL_Hint}.
Further, since annotations are typically added as prefixes or suffixes to SQL statements, the required application modifications are not cumbersome.
We therefore consider this annotation-based mechanism to be reasonable.

We have revised Section \ref{intro} to clarify the novelty of the proposed decentralized prepare mechanism, which allows the prepare phase to begin immediately after the completion of local execution.
Performing decentralized prepare across diverse data sources is challenging due to the varied transaction protocols they employ.
Unlike existing solutions~\cite{DBLP:journals/pvldb/MaiyyaNAA19, DBLP:journals/pvldb/ZhangLZXLXHYD23, DBLP:conf/sosp/ZhangSSKP15, DBLP:conf/usenix/CowlingL12} in distributed database systems, which typically rewrite the transaction protocol, we introduce a non-intrusive and lightweight decentralized prepare mechanism for the middleware system.
We leverage annotations to mark the last read/write operation and develop an efficient component, called geo-agent, to abstract differences between data sources, thereby enabling decentralized preparation across various systems.
In addition, we design an early abort mechanism that allows fault transactions to abort quickly, preventing such transactions from degrading system performance. 
We would like to emphasize that, in addition to the decentralized prepare mechanism, \dbname also incorporates other techniques, i.e., latency-aware scheduling and high-contention optimization, that are novel and cannot be directly achieved through employing annotations.
% We have improved Section~\ref{intro} to clearly articulate the motivation and novelty of the proposed decentralized prepare mechanism and better explain the typical distributed transaction processing protocol.

% In \dbname, we employ these annotations to indicate the last operation in the proposed decentralized prepare mechanism.
% We understand that \dbname requires the users to explicitly notify the database middleware of the last statement by annotation.
% which may be potential invasive application code.
% However, we would like to note that using it is a widely adopted technique in query optimizations in MySQL and PostgreSQL .
% Please refer to our response to R1O1 for more details. 
}

\comments{O2}{
There are several pieces of related work that have different techniques for optimizing distributed transactions and lock contention. For example, QURO and Chiller perform re-ordering, and Carousel integrates the consensus protocol with 2PC. While these papers have different assumptions and are not necessarily middleware. However, a comparison against these systems, which have the same overall goal: reducing distributed transaction overhead, would help contextualize the benefits and trade-offs of GeoTP.
}

\response{O2}{
We have implemented QURO and Chiller within the SSP framework to ensure a fair comparison. For QURO, we modified the application program to reorder read/write operations within a single transaction. For Chiller, one of its optimizations requires rewriting the database kernel to reduce network round trips in distributed transactions, which we achieved using a decentralized prepare mechanism. 
Carousel integrates 2PC with replica consensus to reduce network latency, necessitating extensive protocol modifications in the database kernel. Since \dbname does not involve replica and consensus protocols such as Raft, Carousel's optimization is orthogonal to our contribution, and thus, we did not implement it in the database middleware.
The performance of the other two approaches was evaluated over YCSB and TPC-C benchmarks in Figure \ref{Fig.experiment.ycsb.ds} and Figure \ref{Fig.experiment.tpcc.dis}. The evaluation results indicate that QURO performs better than SSP but falls short compared to other methods. This is primarily because QURO does not account for network latency, making it inadequate for geo-distributed scenarios. 
% Chiller redesigns the protocol to combine the prepare phase into the execution and reduces the lock contention span by executing inner-region subtransactions after the outer-region ones. Its mechanism is similar to \dbname's first two optimizations: decentralized prepare and latency-aware scheduling. However, \dbname outperforms Chiller for two reasons: (1) the Chiller's scheduling is coarse and Not precise enough because it divides nodes as inner and outer regions and Ignores internal differences. (2) \dbname implements specific optimizations for high contention scenarios, enhancing performance. 
Chiller redesigns its protocol by integrating the prepare phase with execution and reducing lock contention by scheduling the intra-region transactions before subtransactions of cross-region transactions. This approach resembles \dbname's partial optimizations: decentralized prepare (O1) and latency-aware scheduling (O2). However, \dbname outperforms Chiller due to two main factors: (1) Chiller's scheduling is imprecise, grouping nodes broadly by intra-regions and cross-regions and missing finer internal distinctions; (2) \dbname incorporates specialized optimizations tailored to high-contention workloads, further improving the performance.
We have revised Section \ref{sec:evaluation_workloads} to provide a deeper analysis of our performance advantages.
}

\comments{O3}{
The paper only briefly discusses GeoTP's overheads, such as the CPU and memory needed to perform tracking contention, build latency models, and maintain the scheduling queue.
}

\response{O3}{
% \begin{figurehere}
%     \centering
%     \begin{subfigure}{0.3\linewidth}
%         \includegraphics[width=\linewidth]{figures/evaluations/revision/cpu.pdf}
%         \vspace{-6mm}
%         \caption{CPU}
%         \label{Fig.revise.stat.cpu}
%     \end{subfigure}
%     \begin{subfigure}{0.3\linewidth}
%         \includegraphics[width=\linewidth]{figures/evaluations/revision/memory.pdf}
%         \vspace{-6mm}
%         \caption{Memory}
%         \label{Fig.revise.stat.mem}
%     \end{subfigure}
%     \begin{subfigure}{0.3\linewidth}
%         \includegraphics[width=\linewidth]{figures/evaluations/revision/breakdown.pdf}
%         \vspace{-6mm}
%         \caption{Breakdown}
%         \label{Fig.revise.stat.breakdown}
%     \end{subfigure}
%     \vspace{-1mm}
%     \caption{Resource Utilization over YCSB}
%     \label{Fig.revise.overhead}
%     \vspace{-5mm}
% \end{figurehere}
We have evaluated the overhead of \dbname from two perspectives: (1) overall system overheads, measured by the CPU utilization and memory usage during the execution phase; and (2) per-transaction overhead, analyzed via a latency breakdown of a distributed transaction.
As shown in Figure \ref{Fig.experiment.overhead}, \dbname improves CPU utilization by 30\% due to the network detection and transaction scheduling, with a memory overhead of 0.3GB for storing metadata on hot records. 
Further, Figure \ref{Fig.stat.breakdown} provides a breakdown of module costs in a transaction lifecycle.
As observed, the analysis time is less than 1 ms, with a 3.5 ms wait time for decentralized preparation before entering the commit phase.
Compared to the entire transaction latency, the overhead incurred by \dbname is negligible, while \dbname achieves 66.6\% lower average transaction latency compared to SSP.
We have revised Section \ref{sec:evaluation_scalability} to include a discussion on the overhead of \dbname. 
% {\color{blue}
% Due to space limitations, we discuss the overhead of \dbname in the extended version of our paper~\cite{GeoTP}. 
% }
}

\comments{O4}{
The deployment architecture is not obvious. Is the middleware layer deployed everywhere the clients are? Does that mean that if there are two data sites, with two sets of clients close to each of the data sites, there will be two instances of the middleware? Will they have opposing scheduling algorithms and defer lock acquisition differently based on the local latency? (Discuss deploying GeoTP with clients in multiple regions)
}

\response{O4}{
\begin{figurehere}
    \centering
    \begin{subfigure}{0.45\linewidth}
        \includegraphics[width=\linewidth]{figures/evaluations/revision/deploy_single.pdf}
        \vspace{-4mm}
        \caption{Single-middleware deployment}
        \label{Fig.revise.deploy.single}
    \end{subfigure}
    \begin{subfigure}{0.45\linewidth}
        \includegraphics[width=\linewidth]{figures/evaluations/revision/deploy_multi.pdf}
        \vspace{-4mm}
        \caption{Multi-middleware deployment}
        \label{Fig.revise.deploy.multi}
    \end{subfigure}
    \caption{Deployment}
    \label{Fig.revise.delpoy}
\end{figurehere}
We would like to clarify that we deploy the middleware on 1 server and the data sources on 4 separate servers, with each server hosting a data source in our experiment, as shown in Figure~\ref{Fig.revise.deploy.single}.
If there are two clients from different regions, they would send requests to the single middleware node.
This deployment plan follows the default deployment of Shardingsphere and existing works~\cite{DBLP:conf/icde/LiZPLWSWCGG22}.
We have improved Section~\ref{sec.evaluation.setup} to make the deployment plan more clear.
% following the default deployment of Shardingsphere and existing works.
% \dbname obeys the deployment of previous database middleware such as Apache Shardingsphere, where a database middleware manages multiple underlying databases and 
% It makes the maintenance work much easier and can mitigate the distributed deadlocks to some extend. 
\begin{figurehere}
    \centering
    \includegraphics[width=0.25\textwidth]{figures/evaluations/revision/multi.pdf}
    % \vspace{-4mm}
    \caption{Clients in multiple regions over YCSB}
    \label{Fig.revise.multi_client}
    \vspace{-4mm}
\end{figurehere}

\dbname can deploy multiple middleware nodes in different regions, as its architecture does not restrict a centralized middleware.
As shown in Figure~\ref{Fig.revise.deploy.multi}, we have deployed two middleware nodes in separate regions and conducted additional experiments to evaluate the performance of \dbname. 
As shown in Figure \ref{Fig.revise.multi_client}, \dbname efficiently scales to multi-region deployment.
Due to space constraints, we chose not to include Figure \ref{Fig.revise.multi_client} in the paper. 
We shall include these experiments in the extended version of our paper~\cite{GeoTP}.
% and the similar conclusion in Figures \ref{Fig.revise.multi_client} and the figures in Section \ref{sec.evaluation},
% Due to the space limitation, we would show the evaluation in our extension version. 
}

\comments{D1}{
The benefit of the early preparation is reduced as the transaction length increases and the number of round trips increases. It would be interesting to conduct experiments with more multi-round transactions.
}

\response{D1}{
We have evaluated the performance of \dbname with increasing network round trips during the execution phase.
As observed in Figure \ref{Fig.experiment.length}, the performance of \dbname decreases by up to 82.1\% as round trips increase from 1 to 6, but it still outperforms the baselines by up to 3.4x. 
Further, we have assessed the performance of \dbname with varying transaction lengths by changing the number of operations in a transaction.
To isolate the impact of transaction length, we ensured that the number of network rounds remained constant in these experiments.
As the transaction length increased from 5 to 25 operations, the performance of \dbname and SSP decreased by 19.1\% and 41.3\%, respectively.
This indicates that network round trips affect \dbname's performance.
However, as stated in our response to R1, most real-world distributed transactions tend to minimize execution round trips for better performance, and standard transactions, such as transferring balance between user accounts and updating user profiles in web applications~\cite{DBLP:conf/sigmod/YangY022, DBLP:conf/sigmod/Pavlo17} require just two rounds for execution~\cite{DBLP:conf/eurosys/ChenSJRLWZCC21}. 
We therefore consider \dbname to be suitable and effective for real-world applications.
We have revised Section \ref{sec:evaluation_length} to analyze the impact of transaction length and interactive rounds. 
% However, transaction length has little impact on our evaluation. 
% query load, workload, 
}

\comments{D2}{I didn't find the evaluation of heterogeneous databases particularly useful; it merely demonstrated that GeoTP supports that deployment.}

\response{D2}{
According to the comment from R2C4, we have improved Section \ref{sec.eva.heterogeneous} to make these experiments focus these experiments on evaluating the performance of different underlying data sources. 
Please refer to our response for R2C4 for more details. 
}

\comments{D3}{What is the accuracy of the models used by GeoTP? How much does this matter? Does a poor estimate of latency result in worse performance?}

\response{D3}{
\begin{figurehere}
    \centering
    \begin{subfigure}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/evaluations/revision/lat_diff_medium.pdf}
        \vspace{-4mm}
        \caption{Medium contention}
        \label{Fig.stat.medium}
    \end{subfigure}
    \begin{subfigure}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/evaluations/revision/lat_diff_high.pdf}
        \vspace{-4mm}
        \caption{High contention}
        \label{Fig.stat.high}
    \end{subfigure}
    \vspace{-1mm}
    \caption{Accuracy of prediction model over YCSB}
    \label{Fig.revise.accuracy}
    \vspace{-4mm}
\end{figurehere}
We propose a heuristic model for latency-aware scheduling. 
To evaluate the accuracy of this model, we collected statistics on the predicted latency and actual latency for the same record (\textit{ycsb\_key = 0}), and then illustrated their difference (predicted latency minus actual execution latency) in Figure \ref{Fig.revise.accuracy}. 
We can observe that in medium contention scenarios, 95.9\% of the differences are within 10 ms, while
% 85.8\% of the differences fall within 5 ms.
% , and 
in high contention scenarios, 82.1\% of the differences are within 10 ms.
% , and 89.2\% transactions fall within 20 ms.  
These results indicate that the heuristic optimization achieves acceptable accuracy.


% , as confirmed by the ablation study. 
We would like to clarify that discrepancies between predicted and actual latency do not always degrade performance.
When the predicted latency is lower than the actual latency, performance may, at worst, revert to that of a system without latency-aware scheduling.
However, if the prediction latency is larger than the actual latency, performance may suffer if the delayed subtransaction becomes the new bottleneck.
In cases of inaccurate runtime predictions, we can scale down the predicted latency before incorporating it into calculations to mitigate any negative impact.
We have revised Section \ref{design-3} to provide more detailed discussions on the impact of inaccurate prediction. 
% Due to the space limitation, we illustrate the accuracy of our heuristic model 
}


% \end{multicols}

% \twocolumn

\clearpage
